Fibrational linguistics: First concepts

We define a general mathematical framework for linguistics based on the theory of fibrations, called FibLang. We start by modelling the interaction between linguistics and cognition in the most general way possible, with a heavy focus on conceptually motivating any assumption we make. The advantage is that FibLang remains agnostic with respect to any particular axiomatization of grammar one may choose. As such, it is compatible with already existing categorical models of language (such as for example, DisCoCat), providing a formally sound framework to apply mathematical tools developed in the context of category theory, mainly categorical logic, to the study of language

==> sections/categorifyingFibrations.tex <==
\section{Categorifying~\autoref{thm:_factorization}}
% \epigraph
% {\textsf{Five card stud, nothing wild, and sky's the limit}}
% {Cpt. Jean-Luc Picard}

Up to now, all the fibrations we consider are \emph{discrete}. This as a somewhat serious limitation to the expressive power of our model, as the elements of meaning over an object $L$ of a language $\clL$ may carry more structure than mere sets (this means: the fibre over a fixed object $L$ can be categories instead than mere sets).

In this section we propose a way to generalise~\autoref{thm:_factorization} to the context of more general fibrations. The price to pay is that a speaker now must be a 2-functor.

Recall that the result sketched in \autoref{stree_fattorizia}, borrowed entirely from \cite{bams1183534973}, establishes a canonical way to factor any given functor $F : \clC \to \clD$ as a discrete fibration $p$ followed by an initial functor $s$:
\[\label{mod_street_fact}\xymatrix{\clC \ar[r]^s & \clE \ar[r]^p & \clD}\]
Now we are interested in a looser kind of factorization theorem, where $p$ is a nondiscrete fibration.%, and we require no property whatsoever on $s$. In particular, we are not interested in requiring that the fibration $p$ is right orthogonal to $s$, but only that the entire procedure has some kind of functoriality.
\begin{proposition}[A Street factorization for non discrete fibrations]\label{modified}
    Every 2-functor $F : \clC \to \clD$ can be factored as a composition \eqref{mod_street_fact} where $p$ is a fibration.
\end{proposition}
% The present argument mimicks the original proof of Street that ensures that the fibration $p$ can be chosen to be discrete.
% For our purposes it is not important what kind of functor $s$ is (if $p$ is discrete, one can show that $s$ is initial, see \cite{bla} and \cite{blo}).
In order to prove \autoref{modified} we have to tweak and dualize the argument given in \cite{bams1183534973}: we need to generalise the construction as follows:
\begin{itemize}
  \item nondiscrete fibres;
  \item contravariant functors.
\end{itemize}
The second goal is easy to achieve: given $F : \clC \to \clD$, just factor \emph{à la Street} the opposite functor $F^\op : \clC^\op \to \clD^\op$ into an initial functor $\clC^\op \to \clE$ followed by an opfibration $p^\op : \clE \to \clD^\op$; $p : \clE^\op \to \clD$ will now be a fibration, factoring $F$.

So, we concentrate on the categorification of \autoref{stree_fattorizia}, showing that it is possible to factor the 2-functor $F : \clC \to \clD$ into a 2-initial functor, followed by an \emph{opfibration} with nondiscrete fibres.

In order to make a guess towards which direction the result can be generalised, it is enough to observe that the left extension
    \[\vcenter{\xymatrix{
      \clC  \ar[d] \ar[r]^F & \clD \ar[d]^{K_F} \\
      {*} \ar[r] & \Set\ultwocell<\omit>{}
    }}\]
used in the proof of \autoref{stree_fattorizia} consists of the functor sending $D\in\clD$ to the colimit of the functor $\clD(F-,D)$, and that the comma object $(*/K_F)$ is the category of elements of $K_F$, thus automatically an opfibration (with fibres the sets $\colim\clD(F-,D)$) --of course, also by virtue of \autoref{lemmacomma}.

\begin{proof}
  If $F$ is a 2-functor, consider the diagram
  % Let $1$ be the terminal category, and $* : 1 \to \Cat$ the functor choosing the terminal category. Consider the functor $K : \clD\to \Cat$ obtained from the right extension
    \[\label{das_komma_quadrat}\vcenter{\xymatrix{
      \clC  \ar[d] \ar[r]^F & \clD \ar[d]^{K_F} \\
      {*} \ar[r] & \Cat\ultwocell<\omit>{}
    }}\]
    where $K$ is the (pointwise) left extension of the terminal functor $\clC \to \Cat$ (constant in the terminal category) along $F$; $K_F$ sends an object $D\in\clD$ to the colimit of the diagram
    \[  X\mapsto\clD(FX,D)\]
    computed in $\Cat$.\footnote{In the comma square \eqref{das_komma_quadrat} an easy computation shows that $K_F$ sends $D\in\clD$ to $\pi_0(F/D)$, the set of connected components of the comma category $(F/D)$; the functor $\var{\elts{\clD}{K}}{\clD}$ is thus just the projection on $D$.}

    By the universal property of the comma objet $(*/K_F)$ we now have a factorization
    \[\vcenter{\xymatrix{
      \clC \ar@/^1pc/[drr]^F\ar@/_1pc/[ddr] \ar[dr]&& \\
      & (*/K) \ar[r]^-p\ar[d] & \clD \ar[d]^{K_F} \\
      & {*} \ar[r] & \Cat\ultwocell<\omit>{}
    }}\]
    and $(*/K)$ is the category of elements of $K_F$, so $p$ is a (non discrete) opfibration over $\clD$.
    % and the comma square
    % \[\vcenter{\xymatrix{
    %   (K/*) \drtwocell<\omit>{} \ar[d] \ar[r] & \clD \ar[d]^K \\
    %   {*} \ar[r] & \Cat
    % }}\]
    % whose universal property ensures that $F$ factors through $(K/*)$ as a composition
    % \[\xymatrix{\clC \ar[r]^-S & (K/*) \ar[r]^-p & \clD}\]
    % it is now a general fact that $p$ is a fibration (cf. \autoref{}).
\end{proof}
